Combinatorial Characterization for Global Identifiability of Separable Networks with Partial Excitation and Measurement

This work focuses on the generic identifiability of dynamical networks with partial excitation and measurement: a set of nodes are interconnected by transfer functions according to a known topology, some nodes are excited, some are measured, and only a part of the transfer functions are known. Our goal is to determine whether the unknown transfer functions can be generically recovered based on the input-output data collected from the excited and measured nodes. We introduce the notion of separable networks, for which global and so-called local identifiability are equivalent. A novel approach yields a necessary and sufficient combinatorial characterization for local identifiability for such graphs, in terms of existence of paths and conditions on their parity. Furthermore, this yields a necessary condition not only for separable networks, but for networks of any topology.

==> archive.tex <==
%==================================================================
%==================================================================
% Wrong proof of proposition on rank \hat K, but the CTDeltaTB
% computation is cool
%==================================================================
%==================================================================

\begin{prop} \label{prop:rank_hat_K_bilidentif}
Exactly one of the two following holds:
	\begin{enumerate}[(i)]
	    \item $\rank \hat K(G) = |E^\Delta|$ for almost all $G$ and $G$ is generically bilinearly identifiable;
		\item $\rank \hat K(G) = |E^\Delta|$ for almost \emph{no} $G$ and $G$ is generically bilinearly non-identifiable.
	\end{enumerate}
\end{prop}

\medskip

\begin{proof}(sketch)\\
    Take $G$ is generically locally bilinearly identifiable\\
    Hence, $\hat G$ is  generically locally identifiable by Proposition \ref{prop:equivalence_bili_decoupled}\\
    So we can apply Proposition \ref{prop:network_identif_rank_condition} on $\hat G$\\
    We compute:
    \begin{align*}
        &\hat C \hat T \hat \Delta \hat T \hat B\\
        &= \begin{bmatrix} C & 0 \\ 0 & 0 \end{bmatrix}
        \begin{bmatrix} T & T\Delta T' \\ 0 & T' \end{bmatrix}
        \begin{bmatrix} 0 & \Delta \\ 0 & 0 \end{bmatrix}
        \begin{bmatrix} T & T\Delta T' \\ 0 & T' \end{bmatrix}
        \begin{bmatrix} 0 & 0 \\ 0 & B \end{bmatrix} \\
        &= \begin{bmatrix} C & CT\Delta T' \\ 0 & 0 \end{bmatrix}
        \begin{bmatrix} 0 & \Delta \\ 0 & 0 \end{bmatrix}
        \begin{bmatrix} 0 & T\Delta T'B \\ 0 & T'B \end{bmatrix}\\
        &= \begin{bmatrix} 0 & CT\Delta T'B \\ 0 & 0 \end{bmatrix}
    \end{align*}
    So we have obtained \eqref{eq:CTDeltaTB_Delta_bili}\\
    Now we can prove that it is equivalent to $\rank \hat K(G) = |E^\Delta|$ by the very same argument as \cite{legat2020local}.
\end{proof}

%==================================================================
%==================================================================
% Notations for section "Conditions"
%==================================================================
%==================================================================

\newg{Notations:}
\begin{itemize}
    \item $n_B:$ nb of excitations, $n_C:$ nb of measures
    \item $|E^\Delta| = n_B n_C:$ nb of unknown edges
    \item $\mathcal{B} = \{b_1 \dots b_{n_B} \}:$ set of excited nodes
    \item $\mathcal{C} = \{c_1 \dots c_{n_C} \}:$ set of measured nodes
    \item $E^\Delta = \{\alpha_1 \dots \alpha_{n_B n_C} \}:$ set of unknown edges
    \item $\sigma:$ Bijection between the unknown edges and the (excitation, measure) pairs
    $$\sigma: E^\Delta \rightarrow \mathcal{B} \times \mathcal{C}: \alpha \rightarrow \sigma(\alpha) = \prt{\sigma_B(\alpha), \sigma_C(\alpha)} = (b, c)$$
    \item $S:$ set of all possible bijections $\sigma$
    \item $\sigma_B:$ Functions between the unknown edges and the excitations. Each excitation is assigned to $n_C$ unknown edges.
    $$\sigma_B: E^\Delta \rightarrow \mathcal{B}: \alpha \rightarrow \sigma_B(\alpha) = b$$
    \item $\sigma_C:$ Functions between the unknown edges and the measures. Each measure is assigned to $n_B$ unknown edges.
    $$\sigma_C: E^\Delta \rightarrow \mathcal{C}: \alpha \rightarrow \sigma_C(\alpha) = c$$
    \item A $\sigma$ is a combination of a $\sigma_B$ and a $\sigma_C$, but not all $(\sigma_B, \sigma_C)$ yield a valid $\sigma$: each pair $(b, c)$ must be assigned to one and only one unknown edge.
    \item $S_B^{\sigma_C}:$ set of all $\sigma_B$ compatible with $\sigma_C$
    \item $S_C^{\sigma_B}:$ set of all $\sigma_C$ compatible with $\sigma_B$
    \item $\sigma_B^{-1}(b):$ set of edges assigned to excitation $b$ in assignation $\sigma_B$. It is of size $n_C$
    \item $\sigma_C^{-1}(c):$ set of edges assigned to measure $c$ in assignation $\sigma_C$. It is of size $n_B$
\end{itemize}

\bigskip

%==================================================================
%==================================================================
% Proof of Proposition \ref{prop:equivalence_bili_decoupled}
%==================================================================
%==================================================================

\medskip

\begin{proof}
    The definition of identifiability on the decoupled network $\hat G$ gives
    \begin{align*}
        \hat C (I- \hat {\tilde G})^{-1} \hat B = \hat C (I- \hat G)^{-1} \hat B
        \Rightarrow \hat {\tilde G}^\Delta = \hat G^\Delta 
    \end{align*}
    for all $\hat {\tilde G}$ consistent with the graph and the known transfer functions, i.e. $\tilde G = G$ and $\tilde G' = G'$. Express the decoupled matrices $\hat C, \hat G, \hat B$ in terms of $C,G, G^\Delta, G',B$ as in Definition \ref{def:decoupled_network}. The closed-loop transfer matrices are given by \eqref{eq:develop_CTB_decoupled}, which yields:
    \begin{align*}
        \begin{bmatrix}
        0 & C \tilde T \tilde G^\Delta \tilde T'B \\
        0 & 0
    \end{bmatrix}
    = \begin{bmatrix}
        0 & CT G^\Delta T'B \\
        0 & 0
    \end{bmatrix}
    \Rightarrow \tilde G^\Delta = G^\Delta 
    \end{align*}
    Since $\tilde G = G$ and $\tilde G' = G'$, we have $(I-\tilde G)^{-1} = (I-G)^{-1}$ and $(I-\tilde G')^{-1} = (I-G')^{-1}$, and we get
    \begin{align*}
        C T \tilde G^\Delta T'B
        = CT G^\Delta T'B
        \Rightarrow \tilde G^\Delta = G^\Delta 
    \end{align*}
    for all $\tilde G^\Delta$ consistent with $G^\Delta$.
    Rearranging the terms gives
    \begin{align*}
        C T (\tilde G^\Delta - G^\Delta) T'B = 0
        \Rightarrow \tilde G^\Delta -G^\Delta =0
    \end{align*}
    Denoting $G^\Delta -G^\Delta$ as $\Delta$ yields expression \eqref{def:decoupled_identif} of Definition \ref{def:decoupled_identif}.
\end{proof}


%==================================================================
%==================================================================
% 3 excitations, 2 measures and 6 edges network :
%==================================================================
%==================================================================

\begin{figure}
	\centering
	\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=2cm,line width=0.3mm,
	minimum size=1mm, % diameter of nonstate nodes
	state/.style={circle, minimum size=3mm}]
	  \node (al)						    {};
	  \node (ar) [right of = al]			{};
	  \node (bl) [below = 5 mm of al]		{};
	  \node (br) [right of = bl]			{};
	  \node (cl) [below = 5 mm of bl]		{};
	  \node (cdl)[below = 2.5 mm of cl]		{};
	  \node (cr) [right of = cl]			{};
	  \node (dl) [below = 5 mm of cl]		{};
	  \node (dr) [right of = dl]			{};
	  \node (el) [below = 5 mm of dl]		{};
	  \node (er) [right of = el]			{};
	  \node (fl) [below = 5 mm of el]		{};
	  \node (fr) [right of = fl]			{};
	  \node[state] (N1) [left of=al] 	  {1};
	  \node[state] (N2) [left of=cdl] 	  {2};
	  \node[state] (N3) [left of=fl] 	  {3};
	  \node[state] (N4) [right of=br] 	  {4};
	  \node[state] (N5) [right of=er] 	  {5};
	  \path (al) edge  node {} (ar)
	  		(bl) edge  node {} (br)
			(cl) edge  node {} (cr)
			(dl) edge   node {} (dr)
			(el) edge   node {} (er)
			(fl) edge   node {} (fr)
	 	   	(N1) edge  node {} (al)
			(N1) edge  node {} (bl)
			(N2) edge  node {} (cl)
			(N2) edge  node {} (dl)
			(N3) edge  node {} (el)
			(N3) edge  node {} (fl)
			(ar) edge  node {} (N4)
			(br) edge node {} (N5)
			(cr) edge node {} (N4)
			(dr) edge node {} (N5)
			(er) edge  node {} (N4)
			(fr) edge  node {} (N5);
	\end{tikzpicture}
	\caption{}
	\label{fig:2E2M}
\end{figure}
